Phase noise characterisation of a 2-km Hollow-Core Nested Antiresonant Nodeless Fibre for Twin-Field Quantum Key Distribution

The performance of quantum key distribution (QKD) is heavily dependent on the physical properties of the channel over which it is executed. Propagation losses and perturbations in the encoded photons' degrees of freedom, such as polarisation or phase, limit both the QKD range and key rate. The maintenance of phase coherence over optical fibres has lately received considerable attention as it enables QKD over long distances, e.g., through phase-based protocols like Twin-Field (TF) QKD. While optical single mode fibres (SMFs) are the current standard type of fibre, recent hollow core fibres (HCFs) could become a superior alternative in the future. Whereas the co-existence of quantum and classical signals in HCF has already been demonstrated, the phase noise resilience required for phase-based QKD protocols is yet to be established. This work explores the behaviour of HCF with respect to phase noise for the purpose of TF-QKD-like protocols. To achieve this, two experiments are performed. The first, is a set of concurrent measurements on 2 km of HCF and SMF in a double asymmetric Mach-Zehnder interferometer configuration. The second, uses a TF-QKD interferometer consisting of HCF and SMF channels. These initial results indicate that HCF is suitable for use in TF-QKD and other phase-based QKD protocols.

==> 202210_SPIEPhotonex_HCF/Extras.tex <==
%this would go into supplementary
\begin{comment}
\begin{figure}
\captionsetup{width=.8\linewidth}
\centering \includegraphics[width=0.9\linewidth]{Figures/PSD w sound}
\caption{\label{Fig_200kSs_Trace} \SA{Voltage power spectral density of the SMF and HCF 2~km spoolsand a power spectral density plot of the ambient sound within the laboratory. All PSD's are processed using Welch's method with a Hann window, width $1\times 10^6$ samples for the SMF and HCF and width $1\times 10^5$ samples for the sound.
}}
\end{figure}
\end{comment}


==> Extras.tex <==
%this would go into supplementary
\begin{comment}
\begin{figure}
\captionsetup{width=.8\linewidth}
\centering \includegraphics[width=0.9\linewidth]{Figures/PSD w sound}
\caption{\label{Fig_200kSs_Trace} \SA{Voltage power spectral density of the SMF and HCF 2~km spoolsand a power spectral density plot of the ambient sound within the laboratory. All PSD's are processed using Welch's method with a Hann window, width $1\times 10^6$ samples for the SMF and HCF and width $1\times 10^5$ samples for the sound.
}}
\end{figure}
\end{comment}

